Multimodal Transfer Deep Learning with Applications in Audio-Visual Recognition

We propose a transfer deep learning (TDL) framework that can transfer the knowledge obtained from a single-modal neural network to a network with a different modality. Specifically, we show that we can leverage speech data to fine-tune the network trained for video recognition, given an initial set of audio-video parallel dataset within the same semantics. Our approach first learns the analogy-preserving embeddings between the abstract representations learned from intermediate layers of each network, allowing for semantics-level transfer between the source and target modalities. We then apply our neural network operation that fine-tunes the target network with the additional knowledge transferred from the source network, while keeping the topology of the target network unchanged. While we present an audio-visual recognition task as an application of our approach, our framework is flexible and thus can work with any multimodal dataset, or with any already-existing deep networks that share the common underlying semantics. In this work in progress report, we aim to provide comprehensive results of different configurations of the proposed approach on two widely used audio-visual datasets, and we discuss potential applications of the proposed approach.

==> MMML %40 NIPS 2015 (TDL) Submission (arXiv)/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Learning from Multimodal Data}
\label{subsec:related_work_multimodal}

Several studies have shown that leveraging multiple modalities for a single shared task often improves the target task, when the parallel multimodal datasets are combined and mutually learned. For instance, \cite{huiskes2010new} showed that using natural language captions or tags in addition to their corresponding standard low-level image features significantly improves classification accuracy of Support Vector Machines (SVM) and Linear Discriminant Analysis (LDA) models. \cite{guillaumin2010multimodal} proposed the multiple kernel learning framework, which showed that an additional text modality can improve the accuracy of SVMs on various object recognition tasks. \cite{xing2012mining} proposed a dual-wing harmonium model to build a joint model of images and text in the latent topic spaces. However, it has been often reported that it is difficult to model multimodal dataset using shallow models, because multimodal data typically has very different statistical properties within different modalities.

Recently, \cite{Ngiam+11a, Ngiam+11b} proposed a deep neural network that can learn features from multiple modalities and predict patterns of single or multiple modalities. Their network composes of a shared representation that takes as input the learned output for each of the two audio and video models, which is then used to make final predictions. Another work by \cite{srivastava2012multimodal} proposes a Deep Boltzman Machine (DBM) for learning multimodal representations of data, where the fused representation is inferred via alternating Gibbs sampling methods. While this line of work shows that the multiple modalities can be combined to improve the performance, most of the work assume the availability of the abundant parallel corpora of different modalities, which is often resource-consuming to obtain. Therefore, our approach addresses this issue by allowing for transfer between data from different modalities.

\subsection{Transfer Learning}
\label{subsec:related_work_transfer_learning}

Transfer learning aims to leverage the knowledge learned from source tasks to perform target tasks which are often provided with limited training resources. Some of the most notable work in this field include the work by \cite{Rosenstein+05, Raina+06, Taylor+07, Mihalkova+08, Yang+11}, most of which study efficient feature or model transfer within different datasets of the same domain. However, applying transfer learning on multimodal datasets where each modality exhibits a completely different sample distribution is known to be extremely challenging, thus traditional transfer learning approaches yield only a small improvement (\cite{Navarretta+13}). As such, instead of performing the feature transfer in the input space or applying the direct model transfer, we perform semantics-level knowledge transfer where only the abstracted features (final computation output of the neural network model) get transferred to each modality. This not only allows for a more robust knowledge transfer, but also entails practical benefits in neural network operations. For example, the transferred data can be directly used in fine-tuning the target model, or performing top-down inference (\cite{Lee+09}) to reconstruct the counterpart modality of the transferred data. \cite{Pan+10} provides a more detailed and comprehensive survey on this topic.

\textbf{Our Contributions}: we summarize our contributions as follows. We propose a novel transfer deep learning (TDL) framework where mapping between abstract representations of different modalities is learned. We propose a set of neural network operations that make use of the transferred knowledge in fine-tuning the target network with the transferred source data. We provide comprehensive empirical results on two multimodal audio-visual datasets using various embedding transfer methods, and show that our approach successfully improves upon the unimodal baseline.



==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Learning from Multimodal Data}
\label{subsec:related_work_multimodal}

Several studies have shown that leveraging multiple modalities for a single shared task often improves the target task, when the parallel multimodal datasets are combined and mutually learned. For instance, \cite{huiskes2010new} showed that using natural language captions or tags in addition to their corresponding standard low-level image features significantly improves classification accuracy of Support Vector Machines (SVM) and Linear Discriminant Analysis (LDA) models. \cite{guillaumin2010multimodal} proposed the multiple kernel learning framework, which showed that an additional text modality can improve the accuracy of SVMs on various object recognition tasks. \cite{xing2012mining} proposed a dual-wing harmonium model to build a joint model of images and text in the latent topic spaces. However, it has been often reported that it is difficult to model multimodal dataset using shallow models, because multimodal data typically has very different statistical properties within different modalities.

Recently, \cite{Ngiam+11a, Ngiam+11b} proposed a deep neural network that can learn features from multiple modalities and predict patterns of single or multiple modalities. Their network composes of a shared representation that takes as input the learned output for each of the two audio and video models, which is then used to make final predictions. Another work by \cite{srivastava2012multimodal} proposes a Deep Boltzman Machine (DBM) for learning multimodal representations of data, where the fused representation is inferred via alternating Gibbs sampling methods. While this line of work shows that the multiple modalities can be combined to improve the performance, most of the work assume the availability of the abundant parallel corpora of different modalities, which is often resource-consuming to obtain. Therefore, our approach addresses this issue by allowing for transfer between data from different modalities.

\subsection{Transfer Learning}
\label{subsec:related_work_transfer_learning}

Transfer learning aims to leverage the knowledge learned from source tasks to perform target tasks which are often provided with limited training resources. Some of the most notable work in this field include the work by \cite{Rosenstein+05, Raina+06, Taylor+07, Mihalkova+08, Yang+11}, most of which study efficient feature or model transfer within different datasets of the same domain. However, applying transfer learning on multimodal datasets where each modality exhibits a completely different sample distribution is known to be extremely challenging, thus traditional transfer learning approaches yield only a small improvement (\cite{Navarretta+13}). As such, instead of performing the feature transfer in the input space or applying the direct model transfer, we perform semantics-level knowledge transfer where only the abstracted features (final computation output of the neural network model) get transferred to each modality. This not only allows for a more robust knowledge transfer, but also entails practical benefits in neural network operations. For example, the transferred data can be directly used in fine-tuning the target model, or performing top-down inference (\cite{Lee+09}) to reconstruct the counterpart modality of the transferred data. \cite{Pan+10} provides a more detailed and comprehensive survey on this topic.

\textbf{Our Contributions}: we summarize our contributions as follows. We propose a novel transfer deep learning (TDL) framework where mapping between abstract representations of different modalities is learned. We propose a set of neural network operations that make use of the transferred knowledge in fine-tuning the target network with the transferred source data. We provide comprehensive empirical results on two multimodal audio-visual datasets using various embedding transfer methods, and show that our approach successfully improves upon the unimodal baseline.


